Indirect Variational Inference: Applications to Earnings Dynamics

Latent-variable models are central to economics but often entail intractable integration. Variational inference (VI), widely used in machine learning, turns this integration into tractable, differentiable optimization by replacing the likelihood with a variational objective. However, guarantees of recovering the true parameters remain limited when the variational family is insufficiently flexible -- a key obstacle to the adoption of VI in economics. We first evaluate VI in models of earnings dynamics and show that the choice of variational posterior is crucial. We then introduce indirect variational inference (IVI), which treats VI as an auxiliary model and corrects the bias induced by the variational approximation. IVI retains much of VI's tractability because it does not require computing the likelihood. We apply these methods to models allowing for nonlinear persistence, non-Gaussian and serially correlated transitory shocks, and latent heterogeneity. Across simulated and empirical applications, flexible variational families combined with IVI deliver reliable estimates.

==> figures/psid_hetro_comp_parameter_table.tex <==
\begin{table}[!t]
\centering
\caption{Estimates on the PSID: Heterogeneous Mean vs.\ Heterogeneous Variance}
\label{psid_hetro_comp_parameter_table}
\setlength{\tabcolsep}{4pt}%
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccc}
\toprule
 & \multicolumn{3}{c}{$\mu(z_{t-1})$} & \multicolumn{3}{c}{$\sigma(z_{t-1})$} & \multicolumn{3}{c}{$f_\alpha(z_1)$} & \multicolumn{3}{c}{$p(a)$} & \multicolumn{3}{c}{$\psi_\gamma(\varepsilon)$} & \multicolumn{1}{c}{$\mathrm{MA}(1)$} \\
\cmidrule(l{2pt}r{2pt}){2-4}\cmidrule(l{2pt}r{2pt}){5-7}\cmidrule(l{2pt}r{2pt}){8-10}\cmidrule(l{2pt}r{2pt}){11-13}\cmidrule(l{2pt}r{2pt}){14-16}\cmidrule(l{2pt}r{2pt}){17-17}
Parameter & $\mu_0$ & $\mu_1$ & $\mu_2$ & $\sigma_0$ & $\sigma_1$ & $\sigma_2$ & $\alpha_1$ & $\alpha_2$ & $\alpha_3$ & $\lambda_0$ & $\lambda_1$ & $\sigma_a$ & $\gamma_1$ & $\gamma_2$ & $\gamma_3$ & $\zeta$ \\
\midrule
\multicolumn{17}{l}{\textit{Heterogeneity in the mean}} \\
(1) unrestr.\ Gaussian (IVI) & $\phantom{-}0.00$ & $\phantom{-}0.98$ & $\phantom{-}0.04$ & $-2.23$ & $-0.16$ & $\phantom{-}0.76$ & $\phantom{-}0.12$ & $\phantom{-}0.57$ & $-0.12$ & $\phantom{-}0.01$ & -- & $\phantom{-}0.16$ & $\phantom{-}0.02$ & $\phantom{-}0.41$ & $-0.08$ & $\phantom{-}0.27$ \\
\addlinespace
\multicolumn{17}{l}{\textit{Heterogeneity in the variance}} \\
(2) unrestr.\ Gaussian (IVI) & $\phantom{-}0.00$ & $\phantom{-}1.00$ & $\phantom{-}0.03$ & $-2.44$ & $-0.14$ & $\phantom{-}0.75$ & $\phantom{-}0.18$ & $\phantom{-}0.68$ & $-0.11$ & $-2.83$ & $-0.18$ & $\phantom{-}0.58$ & $\phantom{-}1.00$ & $\phantom{-}0.62$ & $-0.14$ & $\phantom{-}0.26$ \\
\bottomrule
\end{tabular}%
}
\\ \vspace{0.2cm} \figurenote{The table compares two specifications of individual heterogeneity in the nonlinear earnings model on the PSID, 1980--1989 ($N=741$, $T=10$), each under the IVI-corrected unrestricted-Gaussian variational posterior. In the heterogeneous mean model the individual effect enters additively, $y_t = z_t + a + \varepsilon_t$, with $a \sim \mathcal{N}(\lambda_0, \sigma_a^2)$ independent of $z_1$; in the heterogeneous variance model it enters as a log-scale of the transitory component, $e^{a}\varepsilon_t$, with $a\,|\,z_1 \sim \mathcal{N}(\lambda_0+\lambda_1 z_1, \sigma_a^2)$. Here $\mu(z_{t-1})$ and $\sigma(z_{t-1})$ are the conditional mean and volatility of the persistent state, $f_\alpha(z_1)$ the initial-state law, $\psi_\gamma(\varepsilon)$ the transitory law (scale $\gamma_1$, tail $\gamma_2$, skewness $\gamma_3$), and $\zeta$ the MA(1) coefficient. The transitory scale $\gamma_1$ equals one by construction in the heterogeneous variance model.}
\end{table}

